In-Context Learning for Few-Shot Molecular Property Prediction

In-context learning has become an important approach for few-shot learning in Large Language Models because of its ability to rapidly adapt to new tasks without fine-tuning model parameters. However, it is restricted to applications in natural language and inapplicable to other domains. In this paper, we adapt the concepts underpinning in-context learning to develop a new algorithm for few-shot molecular property prediction. Our approach learns to predict molecular properties from a context of (molecule, property measurement) pairs and rapidly adapts to new properties without fine-tuning. On the FS-Mol and BACE molecular property prediction benchmarks, we find this method surpasses the performance of recent meta-learning algorithms at small support sizes and is competitive with the best methods at large support sizes.

==> sections/approach.tex <==
We propose a method to group tasks by examining the effect to which one task's gradient would increase or decrease another task's loss. We formally define the method in \Secref{sec:algorithm}, describe a systematic procedure to go from inter-task affinity scores to a grouping of tasks in \Secref{sec:network_selection}, and provide theoretical analysis in \Secref{sec:theory}. 

\subsection{Inter-Task Affinity}
\label{sec:algorithm}
Within the context of a hard-parameter sharing paradigm, tasks collaborate to build a shared feature representation which is then specialized by individual task-specific heads to output a prediction. Specifically, through the process of successive gradient updates to the shared parameters, tasks implicitly transfer information to each other. As a consequence, we propose to view the extent to which a task's successive gradient updates on the shared parameters affect the objective of other tasks in the network as a proxy measurement of inter-task affinity.

Consider a multitask loss function parameterized by $\{\theta_s\}\cup \{\theta_i\vert\, i \in \T\}$ where $\theta_s$ represents the shared parameters and $\theta_i$ represents the task $i\in \T$ specific parameters.
Given a batch of examples $\mathcal{X}$, let

\vspace{-0.9cm}
\begin{align*}
    L_{\total}(\mathcal{X}, \theta_{s}, \{\theta_{i}\}) = \sum_{i \in \T} L_{i}(\mathcal{X}, \theta_{s}, \theta_{i})\, ,
\end{align*}
denote the total loss where $L_i$ represents the non-negative loss of task $i$. For simplicity of notation, we set the loss weight of each task to be equal to 1, though our construction generalizes to arbitrary weightings.

For a given training batch $\mathcal{X}^t$ at time-step $t$, define the quantity $\theta_{s\vert i}^{t+1}$ to represent the updated shared parameters after a gradient step with respect to the task $i$. Assuming stochastic gradient descent for simplicity, we have
\vspace{-0.4cm}
\begin{align*}
    \theta_{s\vert i}^{t+1} \coloneqq \theta_{s}^{t} - \eta \nabla_{\theta_s^t}L_i(\mathcal{X}^t, \theta_s^t, \theta_i^t)\, .
\end{align*}
We can now calculate a \textit{lookahead} loss for each task by using the updated shared parameters while keeping the task-specific parameters as well as the input batch unchanged.
That is, in order to assess the effect of the gradient update of task $i$ on a given task $j$, we can compare the loss of task $j$ before and after applying the gradient update from task $i$ onto the shared parameters. 
To eliminate the scale discrepancy among different task losses, we consider the ratio of a task's loss before and after the gradient step on the shared parameters as a scale invariant measure of relative progress. We can then define an asymmetric measure for calculating the \emph{affinity} of task $i$ at a given time-step $t$ on task $j$ as 
\begin{align}
    \label{eq:Z-alpha}
    \mathcal{Z}^t_{i \shortarrow j} = 1 - \frac{L_{j}(\mathcal{X}^t, \theta_{s\vert i}^{t+1}, \theta_{j}^{t})}{L_{j}(\mathcal{X}^t, \theta_s^t, \theta_j^t)}\, .
\end{align}
Notice that a positive value of $\affinity{i}{j}$ indicates that the update on the shared parameters results in a lower loss on task $j$ than the original parameter values, while a negative value of $\mathcal{Z}^t_{i \shortarrow j}$ indicates that the shared parameter update is antagonistic for this task's performance. Our suggested measure of inter-task affinity is computed at a per-step level of granularity, but can be averaged across all steps, every $n$ steps, or a contiguous subset of steps to derive a ``training-level'' score:
\begin{equation*}
    \avgaffinity{i}{j} = \frac{1}{T} \sum_{t=1}^{T} \mathcal{Z}^t_{i \shortarrow j}\, .
\end{equation*}
In \Secref{sec:expts}, we find $\avgaffinity{i}{j}$ is empirically effective in selecting high performance task groupings and provide an ablation study along this dimension in \Secref{sec:ablations}. 

\subsection{Network Selection Algorithm}
\label{sec:network_selection}
At a high level, our proposed approach trains all tasks together in one model, measures the pairwise task affinities throughout training, identifies task groupings that maximize total inter-task affinity, and then trains the resulting groupings for evaluation on the test set. We denote this framework as {\color{modelpink} \mbox{Task Affinity Grouping (TAG)}} and now describe the algorithm to convert inter-task affinity scores into a set of multi-task networks. More formally, given $\binom{|\mathcal{T}|}{2}$ values representing the pairwise inter-task affinity scores collected during a single training run, our network selection algorithm should produce $k$ multi-task networks, $k \leq b$ where $b$ is the inference-time memory budget, with the added constraint that every task must be served from exactly one network at inference.   

For a group composed of a pair of tasks $\{a,b\}$, the affinity score onto task $a$ would simply be $\avgaffinity{b}{a}$ and the affinity score onto task $b$ would be $\avgaffinity{a}{b}$. For task groupings consisting of three or more tasks, we approximate the inter-task affinity onto a given task by averaging the pairwise affinities onto this given task. Consider the group consisting of tasks $\{a, b, c\}$. We can compute the total inter-task affinity onto task $a$ by averaging the pair-wise affinities from tasks $b$ and $c$ onto $a$:  $\sfrac{(\avgaffinity{b}{a} + \avgaffinity{c}{a})}{2}$.

After approximating higher-order affinity scores for each network consisting of three or more tasks, we select a set of $k$ multi-task networks such that the total affinity score onto each task used during inference is maximized. Informally, each task that is being served at inference should train with the tasks which most decrease its loss throughout training. This problem is NP-hard (reduction from Set-Cover) but can be solved efficiently with a branch-and-bound-like algorithm as detailed in \cite{standley2019tasks} or with a binary integer programming solver as done by \cite{taskonomy}. 

\subsection{Theoretical Analysis}
\label{sec:theory}
We now offer a theoretical analysis of our measure of inter-task affinity. Specifically, our goal is to provide an answer to the following question: given that task $b$ induces higher inter-task affinity than task $c$ on task $a$,  does training $\{a,b\}$ together result in a lower loss on task $a$ than training $\{a,c\}$? Intuitively, we expect the answer to this question to always be positive. However, it is easy to construct  counter examples for simple quadratic loss functions where training $\{a, b\}$ actually induces a higher loss than training $\{a, c\}$ (see Appendix). Nonetheless, we show that in a convex setting and under some mild assumptions, the grouping suggested by our measure of inter-task affinity must induce a lower loss value on task $a$.

For simplicity of notation, we ignore the task specific parameters and use $L_a(\theta)$ to denote the loss of task $a$ evaluated at shared parameters $\theta$. Additionally, we denote the gradient of tasks $a$, $b$, and $c$ at $\theta$ as $g_a$, $g_b$, and $g_c$, respectively.
\begin{restatable}{lemma}{lemmainner}
\label{lemma:inner_product}
Let $L_a$ be a $\alpha$-strongly convex and $\beta$-strongly smooth loss function. Given that task $b$ induces higher inter-task affinity than task $c$ on task $a$, the following inequality holds:
\begin{equation}
\label{eq:adotb}
g_a \cdot g_c - \frac{\beta\,\eta}{2}\,\Vert g_c\Vert^2 + \frac{\alpha\,\eta}{2}\,\Vert g_b\Vert^2\leq g_a \cdot g_b  
\end{equation}
\end{restatable}
The proof is given in the Appendix.
\begin{restatable}{proposition}{propmain}
\label{prop:main}
Let $L_a$ be a $\alpha$-strongly convex and $\beta$-strongly smooth loss function. Let $\eta \leq \frac{1}{\beta}$ be the learning rate. Suppose that in a given step, task $b$ has higher inter-task affinity than task $c$ on task $a$. Moreover, suppose that the gradients have equal norm, i.e. $\Vert g_a\Vert = \Vert g_b\Vert = \Vert g_c\Vert$. Then, taking a gradient step on the parameters using the combined gradient of $a$ and $b$ reduces $L_a$ more so than taking a gradient step on the parameters using the combined gradient of $a$ and $c$, given that $\cos(g_a, g_c) \leq \frac{\eta}{4} \frac{\alpha\, \beta}{\beta - \alpha} - 1
$ where $\cos(u, v) \coloneqq \frac{u \cdot v}{\Vert u\Vert\, \Vert v\Vert}$ is the cosine similarity between $u$ and $v$.
\end{restatable}
The proof is given in the Appendix. Proposition~\ref{prop:main} intuitively implies the grouping chosen by maximizing per-task inter-task affinity is guaranteed to make more progress than any other group. 
Moreover, the assumptions for this condition to hold in the convex setting are fairly mild.
Specifically, our first assumption relies on the gradients to have equal norms, but our proof can be generalized to when the gradient norms are approximately equal. 
This is often the case during training when tasks use similar loss functions and/or compute related quantities. 
The second assumption relies on the cosine similarity between the lower-affinity task $c$ and the primary task $a$ being smaller than a constant.
This is a mild assumption since the ratio $\frac{\sfrac{\beta}{\alpha}}{\sfrac{\beta}{\alpha} - 1}$ becomes sufficiently large for the assumption to hold trivially when the Hessian of the loss has a sufficiently small condition number.

